Clifford algebra and the projective model of Hyperbolic spaces

I apply the algebraic framework developed in [1] to study geometry of hyperbolic spaces in 1, 2, and 3 dimensions. The background material on projectivised Clifford algebras and their application to Cayley-Klein geometries is described in [2].

==> g-1.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887808,113.958449)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-85.376640,221.199366)(0.000000,-0.360142){$H_1$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-90.776640,139.585075)(-1.000000,-0.250000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-90.776640,102.216267)(-1.000000,-0.750000){$\textbf{b}$}


==> g-10.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-10_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-146.776131,102.778441)(-1.000000,-0.625000){$\textbf{N}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-106.011694,103.642246)(0.000000,0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-118.324680,132.546726)(0.000000,0.000000){$S\textbf{P}S^{-1}$}


==> g-11+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-11+0_0.pdf}%
}%


==> g-11.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-11+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-11+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-11+0.prc}}


==> g-12+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-12+0_0.pdf}%
}%


==> g-12.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 226.238490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,113.119245)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-12+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.847616332356153634,3Droll=0,3Droo=410.847616332356153634,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-12+0.js]{254.9525pt}{223.83625pt}{\ASYprefix\jobname-12+0.prc}}


==> g-13+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-13+0_0.pdf}%
}%


==> g-13.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 224.231000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.115500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-13+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -408.77568281534882999,3Droll=0,3Droo=408.77568281534882999,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-13+0.js]{254.9525pt}{221.82875pt}{\ASYprefix\jobname-13+0.prc}}


==> g-14+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-14+0_0.pdf}%
}%


==> g-14.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 224.231000pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.115500)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-14+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -408.775682815348943677,3Droll=0,3Droo=408.775682815348943677,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-14+0.js]{254.9525pt}{221.82875pt}{\ASYprefix\jobname-14+0.prc}}


==> g-15+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-15+0_0.pdf}%
}%


==> g-15.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-15+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-15+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-15+0.prc}}


==> g-16+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-16+0_0.pdf}%
}%


==> g-16.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 225.234750pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,112.617375)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-16+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -409.971468858113951228,3Droll=0,3Droo=409.971468858113951228,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-16+0.js]{254.9525pt}{222.8325pt}{\ASYprefix\jobname-16+0.prc}}


==> g-2.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0.pdf}%
}%
\special{pdf:q}%
\begin{picture}( 232.815023, 233.316898)%
\special{pdf:\ASYraw{
 -231.695229 0.500000 m
 -0.250000 0.500000 l
 -0.250000 231.945229 l
 -231.695229 231.945229 l
 -231.695229 0.500000 l
h
W n
}%
}%
\special{pdf:\ASYraw{
 -231.695229 -54.794576 m
 -0.250000 -54.794576 l
 -0.250000 287.239804 l
 -231.695229 287.239804 l
 -231.695229 -54.794576 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.887807,113.958449)(-0.500000,-1.000000){$w$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.107512,229.676408)(-1.000000,-0.500000){$x$}
\end{picture}%
\kern -232.815023pt%
\special{pdf:Q}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-85.376640,221.199366)(0.000000,-0.360142){$H_1$}


==> g-3.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-111.401586,186.500378)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-168.189403,185.292901)(-1.000000,-0.750000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-47.667113,133.035568)(-0.666667,0.226360){$(\textbf{a}\wedge\textbf{b})\textbf{I}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-83.540155,31.481789)(-0.000000,-0.500000){$\textbf{a}\wedge\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-100.532597,110.992691)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-125.949997,102.126474)(-0.750000,-0.779180){$\textbf{Q}$}


==> g-4+0.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4+0_0.pdf}%
}%


==> g-4.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
\leavevmode\vbox to 214.193490pt{}%
\kern 257.354750pt%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-128.677375,107.096745)(-0.500000,-0.500000){\includemovie[3Dlights=File,text={\includegraphics[hiresbb]{\ASYprefix\jobname-4+0_0.pdf}},label=,toolbar=false,3Daac=0,3Dc2c=0 0 1,3Dcoo=0 0 -410.889700647751340057,3Droll=0,3Droo=410.889700647751340057,3Dbg=1 1 1,3Djscript=\ASYprefix\jobname-4+0.js]{254.9525pt}{211.79125pt}{\ASYprefix\jobname-4+0.prc}}


==> g-5.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-151.723356,209.781558)(-1.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-58.692222,143.867271)(0.000000,-1.000000){\textbf{a}\textbf{I}}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-129.671429,124.939482)(0.000000,-1.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-185.804689,108.672512)(-0.366667,-1.000000){$\textbf{a}\cdot\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-107.613942,130.742729)(-0.000000,-0.473640){$(\textbf{P}\cdot\textbf{a})\textbf{a}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-61.054722,147.411021)(-0.750000,0.226360){$(\textbf{P}\wedge\textbf{a})\textbf{a}^{-1}$}


==> g-6.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-6_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-146.323356,209.781558)(0.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-128.017679,129.900732)(-0.125000,-0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-209.781558,158.888876)(-0.500000,0.000000){$\textbf{b}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-84.342128,209.781558)(0.000000,-0.402231){$-\textbf{a}\textbf{b}\textbf{a}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-94.336903,138.976772)(0.000000,0.000000){$\textbf{a}\textbf{P}\textbf{a}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-40.219581,23.532118)(0.000000,-0.500000){$\textbf{c}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-64.864387,23.532118)(-1.000000,-0.402231){$-\textbf{a}\textbf{c}\textbf{a}^{-1}$}


==> g-7.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-7_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-70.239226,46.813298)(-1.000000,-0.500000){$\textbf{a}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-128.962679,126.120732)(-0.000000,-0.500000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-151.139229,46.813298)(0.000000,-0.500000){$\textbf{P}\textbf{a}\textbf{P}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-46.813298,168.373705)(-0.500000,0.115074){$\textbf{P}\textbf{e}_2\textbf{P}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-203.370909,66.893286)(0.000000,-0.833333){$\textbf{P}\textbf{I}^{-1}$}


==> g-8.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-8_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-170.605204,92.045155)(-0.125000,-0.000000){$\textbf{T}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-93.515956,48.020774)(0.000000,-0.250000){$\textbf{T}\textbf{I}^{-1}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-104.357944,106.240996)(-0.125000,-0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.019338,85.902655)(-1.000000,-0.771075){$\textbf{N}_+$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-141.732684,131.329348)(-1.000000,-0.771075){$\textbf{N}_-$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-116.798199,134.079803)(-0.125000,-0.000000){$T\textbf{P}T^{-1}$}


==> g-9.tex <==
\setlength{\unitlength}{1pt}
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-9_0.pdf}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-4.073583,113.956838)(-0.500000,-1.000000){$x$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-119.356838,229.049123)(-1.000000,-0.188888){$y$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-126.127679,110.740167)(-0.000000,-0.375000){$\textbf{R}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-106.011694,103.642246)(0.000000,0.000000){$\textbf{P}$}
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}
\fontsize{9.000000}{10.800000}\selectfont
\ASYalign(-127.107978,133.811234)(0.000000,0.000000){$R\textbf{P}R^{-1}$}

